Metric dimension on sparse graphs and its applications to zero forcing sets

The metric dimension dim(G) of a graph $G$ is the minimum cardinality of a subset $S$ of vertices of $G$ such that each vertex of $G$ is uniquely determined by its distances to $S$. It is well-known that the metric dimension of a graph can be drastically increased by the modification of a single edge. Our main result consists in proving that the increase of the metric dimension of an edge addition can be amortized in the sense that if the graph consists of a spanning tree $T$ plus $c$ edges, then the metric dimension of $G$ is at most the metric dimension of $T$ plus $6c$. We then use this result to prove a weakening of a conjecture of Eroh et al. The zero forcing number $Z(G)$ of $G$ is the minimum cardinality of a subset $S$ of black vertices (whereas the other vertices are colored white) of $G$ such that all the vertices will turned black after applying finitely many times the following rule: a white vertex is turned black if it is the only white neighbor of a black vertex. Eroh et al. conjectured that, for any graph $G$, $dim(G)\leq Z(G) + c(G)$, where $c(G)$ is the number of edges that have to be removed from $G$ to get a forest. They proved the conjecture is true for trees and unicyclic graphs. We prove a weaker version of the conjecture: $dim(G)\leq Z(G)+6c(G)$ holds for any graph. We also prove that the conjecture is true for graphs with edge disjoint cycles, widely generalizing the unicyclic result of Eroh et al.

==> archive.tex <==


\section{Old proof for Theorem \ref{odd_unicyclic}}

\begin{proof}
For the proof we consider the structure of $G$. Recall that the length of the cycle is $2k+1$. The proof is based on a case analysis.

\begin{enumerate}
    \item \textbf{For every $u \in C$, $T_u$ is a rooted tree.} \\ 
    By Lemma~\ref{zero}, there is an edge $e$ such that  $Z(G-e) \leq Z(G)$. Since the $G-e$ is a tree, Corollary~\ref{unicycle} ensures that $\dim(G-e) \leq Z(G-e)$. By Lemma~\ref{tree}, $\dim(G) \leq \dim(G-e)$. The combination of these inequalities gives $\dim(G) \leq Z(G)$.
    
    \item \textbf{For every $u \in C$, $T_u$ is a rooted path.} \\ 
    We claim that any pair of vertices $\alpha$ and $\beta$ of $C$ at distance $k$ is a resolving set. Let ${\alpha,\beta}$ be such a pair of vertices. Let us prove that for every $x \in G$, $d(x,\alpha)+d(x,\beta) \in \{k,k+1\}$ if and only if $x \in C$. Indeed as $d(\alpha,\beta)=k$ for any vertex $x$, $d(x,\alpha)+d(x,\beta) \geq k$. If $x \in C$ either $x$ is on the path between $\alpha$ and $\beta$ and $d(x,\alpha)+d(x,\beta) =k$ or $x$ is in the other part of the cycle and $d(x,\alpha)+d(x,\beta) = k+1$. If $x \notin C$ then let $y$ be the vertex of $C$ such that $x \in T_y$. Then, $d(x,\alpha)+d(x,\beta)=d(y,\alpha)+d(y,\beta)+2d(x,y) \geq 2 +d(y,\alpha)+d(y,\beta) \geq k+2$. This implies that a vertex on the cycle cannot have the same code as a vertex not on the cycle. \\
    As $\alpha$ and $\beta$ are vertices of $C$, Lemma~\ref{cycle} applies. Then two vertices on $C$ cannot have the same code.
    Two vertices not in $C$ cannot have the same code then one of the previous case must apply. Assume by contradiction that two vertices $x$ and $y$ are not resolved by $\{\alpha, \beta\}$ with $x \in T_u$ and $y \in T_v$ for $u$ and $v$ in $C$. If $u=v$ since $T_u$ is a rooted path $\alpha$ resolves the pair $(x,y)$ immediately. Assume from now $u \neq v$. Assume by symmetry $d(x,u) \leq d(y,v)$ and let $z \in T_v$ be the vertex on $T_v$ such that $d(v,z)=d(x,u)$. Then, the pair $\{\alpha,\beta\}$ does not resolve the pair $(z,u)$ but $u \in C$ and the previous cases gives that any pair of vertices with one vertex on $C$ is resolved by $\{\alpha,\beta\}$. We get a contradiction and then pair $\{\alpha,\beta\}$ resolves $G$. So $\dim(G)=2$ and as $G$ is not a path $Z(G) \geq 2$.
    
    \item \textbf{There exists a unique $u \in C$ such that $T_u$ is a rooted tree}.\\ 
    Let us prove that $\dim(G) \leq \dim(T_u)+1$ and $Z(G) \geq Z(T_u)+1$.
    Let $S$ be a basis for $T_u$ and $v \in C$ a vertex at distance $k$ from $u$. Let us show that $S \cup \{v\}$ is a resolving set of $G$. Let $\alpha \in S \cap T_u$, then two vertices in $G \setminus T_u$ cannot have the same distance to $\alpha$ and $v$. Indeed otherwise these two vertices would have the same distance to $u$ and $v$ which is impossible since in $G \setminus T_u$, for every $v \in C$ $T_v$ is a rooted path and by point (2) $\{u,v\}$ is a resolving set. 
    Two vertices on $T_u$ cannot have the same code since $S$ is a basis for $T_u$ and $u$ is a cutvertex.
    Let $x \in T_w$ for some $w \in C$ and $y \in T_u$. By the triangular inequality $d(\alpha,y) \leq d(y,u)+d(u,\alpha)$.
    If $d(\alpha,y)=d(\alpha,x)$ then $d(x,u) \leq d(y,u)$ as $d(\alpha,x)=d(\alpha,u)+d(u,x)$. If $d(x,v)=d(y,v)$ then as $d(y,v)=d(y,u)+d(u,v) \geq d(x,u)+d(u,v)$. We get $d(x,v) \geq d(x,u)+d(u,v)$. Removing $d(x,w)$ on both side gives $d(w,v) \geq d(w,u)+d(u,v)$ which is impossible as $d(u,v)=k$ and $d(w,v) \leq k$. So $x$ and $y$ have different codes and $\dim(G) \leq \dim(T_u)+1$. \\
    Let $Z$ be a minimal zero forcing set of $G$. If $Z$ contains $u$, then it should contain at least another vertex in $G \setminus T_u$. Since the restriction of $Z$ to $T_u$ is a forcing set for $T_u$ we have $Z(G) \geq Z(T_u)+1$. 
    So we can assume that $u \notin Z$. Consider a sequence of color change rule that turns $v$ into black. Either $u$ is forced by a vertex in $G \setminus T_u$ since $(G \setminus T_u) \cup \{u\})$ contains a cycle there are at least two vertices in $Z \cap (G \setminus T_u)$ and $Z \cap T_u  \cup \{u\}$ is a forcing set of $T_u$. So $Z(G) \geq Z(T_u)+1$. Otherwise $u$ is forced by a vertex of $T_u$ then there is at least one vertex in $Z \cap (G \setminus T_u)$ and $Z \cap T_u  $ is a forcing set of $T_u$ so $Z(G) \geq Z(T_u)+1$. So in both cases we have $\dim(G) \leq \dim(T_u)+1 \leq Z(T_u)+1 \leq Z(G)$.
    
    \item \textbf{There exists $w \in C$ such that $T_w$ is a rooted path and there exist two vertices $u$ and $v$ in $C$ such that $T_u$ and $T_v$ are rooted trees.} \\
    We assume by contradiction $\dim(G) > Z(G)$. The proof consists in finding $e \in E(C)$ such that $\dim(G-e) < Z(G-e)$ and $Z(G-e) \leq Z(G)$. We use Lemma~\ref{deg1} to find such an edge and Lemma~\ref{treecomp} to get a contradiction. 
    \begin{enumerate}
        \item \textbf{There exists a component $T_u$ with $\ell_u =0$.}
        \begin{enumerate}
            \item \textbf{There exists $x \in C$ with $\ell_x \geq 1$ and $ux \notin E(C)$.} \\ 
            Let $e$ be an edge incident to $x$ satisfying the conclusion of Lemma~\ref{deg1}. By Lemma~\ref{deg1} $Z(G-e) \leq Z(G)$. And $\dim(G-e) < Z(G-e)$ by Lemma~\ref{treecomp} since $u$ has degree at least three but is not a major vertex with terminal degree greater than 2. So $\dim(G-e) \leq Z(G)+1$ and, by Lemma~\ref{vardim}, $\dim(G) \leq \dim(G-e)+1$ which give the conclusion.
            
            \item \textbf{Now assume that $\ell_v=0$.} \\
            Let $e$ be an edge incident to $w$ satisfying the conclusion of Lemma~\ref{deg1}. The edge $e$ is not incident to $u$ or $v$, assume by symmetry $e$ is not incident to $u$. Then $Z(G-e) \leq Z(G)$ and $\dim(G-e) < Z(G-e)$ by Lemma~\ref{treecomp} since $u$ has degree at least three but is not a major vertex with terminal degree at least $2$. So $\dim(G-e) \leq Z(G)+1$ and by Lemma~\ref{vardim} $\dim(G) \leq \dim(G-e)+1$ which give the conclusion.
            
            \item \textbf{So we can assume that $\ell_v \geq 1$ with $v$ and $x$ incident to $u$ and $T_u,T_v,T_x$ are the only rooted trees of $C$.} \\
            Let $e$ be an edge incident to $v$ satisfying the conclusion of Lemma~\ref{deg1}. Then, $Z(G-e) \leq Z(G)$. If $e=uv$ then $x$ has degree three in $G-e$ but is not a major vertex with terminal degree at least 2 so $\dim(G-e) < Z(G-e)$ by Lemma~\ref{treecomp}. And if $e$ is the other edge of $E(C)$ incident to $v$ then $u$ has degree at least three in $G-e$ but is not a major vertex with terminal degree at least $2$ so $\dim(G-e) < Z(G-e)$ by  Lemma~\ref{treecomp}.
        \end{enumerate}
        \item \textbf{Not all the rooted trees are consecutive.} \\
        Let $w \in C$ be the root of a path. Then, there exist $u,w,v,z$ appearing in this order in the cycle such that $T_u$ and $T_v$ are rooted trees and $T_z$ root of a path. Let $e$ be an edge incident to $w$ satisfying the conclusion of Lemma~\ref{deg1}. Then $Z(G-e) \leq Z(G)$. And $\dim(G-e) < Z(G-e)$ by Lemma~\ref{treecomp} since $z$ is neither a terminal vertex, a major vertex or an interior degree two vertex in $G-e$. So $\dim(G-e) \leq Z(G)+1$ and by Lemma~\ref{vardim} $\dim(G) \leq \dim(G-e)+1$ which give the conclusion.
        \\From now we can assume the rooted trees are consecutive.
        \item \textbf{There are at least three consecutive rooted trees $T_u,T_v,T_w$.} \\ 
        Without loss of generality assume $u$ is adjacent to $v$ and $w$. Let $e$ be an edge incident to $u$ satisfying the conclusion of Lemma~\ref{deg1}. Without loss of generality assume $e=uv$. Then $Z(G-e) \leq Z(G)$. By Lemma~\ref{treecomp} $\dim(G-e) < Z(G-e)$ since the vertex in $C$ incident to $w$ which is not $u$ have degree three in $G-e$ but is not a major vertex with terminal degree at least 2. So $\dim(G-e) \leq Z(G)+1$ and by Lemma~\ref{vardim} $\dim(G) \leq \dim(G-e)+1$ which gives the conclusion.
        \item \textbf{There is exactly two rooted trees $T_u$ and $T_v$} \\
        Recall that $u$ and $v$ are supposed adjacent.
            \begin{enumerate}
                \item  \textbf{Assume first $\ell_u=1$.} \\ 
                Let $e$ be an edge incident to $u$ satisfying the conclusion of Lemma~\ref{deg1}. Then $Z(G-e) \leq Z(G)$. If $e=uv$ then by Lemma~\ref{treecomp} $\dim(G-e) < Z(G-e)$ since of $u$ which has degree at least three but is not a major vertex with terminal degree greater than 2 in $G-e$. If $e=vw$ where $w$ is the other vertex adjacent to $v$ and $\dim(G-e) = Z(G-e)$ then $u$ is a major vertex in $G-e$ so $v$ is also a major vertex. So $v$ is connected to two leaves in $G-e$. As $\ell_v=1$ the deletion of $e$ gives a new terminal vertex to $u$ which can only be the terminal vertex of the path rooted in $w$. That mean there is only one vertex which is root of a path. Let $e'$ be an edge incident to $u$ satisfying the conclusion of Lemma~\ref{deg1} in $G-e'$. with $Z(G-e') \leq Z(G)$. If $e'=uv$ then by Lemma~\ref{treecomp} $\dim(G-e') < Z(G-e')$since $w$ has degree 3 in $G-e'$ and $\ell_w=1$ ($w$ is connected to $u$ and $v$ which are not root of a rooted path). If $e'$ is the other edge incident to $u$ then by Lemma~\ref{treecomp} $\dim(G-e') < Z(G-e')$ because of $u$ which is not a major vertex with terminal degree at least 2 in $G-e'$.
                \item  \textbf{$\ell_u \geq 2$ and $l_v \geq 2$.}\\
                Let $e=uv$ we have $Z(G-e) \leq Z(G)$. Let $Z$ be a minimum forcing set of $G$ then in $Z \cap T_u$ there is a vertex in a path from $u$ to a terminal vertex. We can assume this vertex is the terminal vertex and force all the path until $u$. Same for $v$ so $e$ is not used to forced any vertex. 
                By Lemma~\ref{treecomp} $\dim(G-e) < Z(G-e)$ because of one vertex root of a path which is not a major vertex with terminal degree greater than 2 in $G-e$. \qedhere
            \end{enumerate}
    \end{enumerate}
\end{enumerate}
\end{proof}
\section{General bound}\

The goal of this section is the prove the following theorem:

\begin{theorem}\label{main}
Let $G=(V,E)$ be a graph of cycle rank at least one. Then, $\dim(G) \leq  Z(G) + \min(5c(G)+\tau(G)-5,3c(G)+5\tau(G)-5)$.
\end{theorem}

Since $\tau(G)\leq c(G)$, we obtain the following linear bound:

\begin{cor}\label{bornec}
For any graph $G$ of cycle rank at least one, $\dim(G) \leq Z(G)+ 6c(G)-5$.
\end{cor}

\subsection{Outline of the proof of Theorem \ref{main}}
The result is known if $c(G) \leq 1$, hence in the rest of the proof we will consider a graph $G$ with $c(G)\geq 2$. The main idea of the proof of Theorem \ref{main} is to remove a small number of vertices in order to guarantee that the resulting connected components $T$ are trees with nice properties. We then use the inequality $\dim(T) \leq Z(T)$ on these trees. We finally prove that the size of a resolving set cannot increase too much and the size of a zero forcing set cannot reduce too much when we return to $G$. Slightly more formally, we will do the following.
\begin{enumerate}
    \item Find a (small) set of vertices $M$ such that: (1) $M$ contains a feedback vertex set $X$, (2) $G \setminus M$ is a forest and, (3) each connected component $H$ of $G\setminus M$  is connected to at most two vertices of $M$ (Lemma~\ref{structure}).
    \item Define a (small) set of vertices $P$ that  identify in which connected component $H$ of $G \setminus M$ a vertex belongs to (Lemma~\ref{use_of_p}).
    \item For each connected component $G_i$ of $G \setminus X$, let $S_{G_i}$ be a metric basis of $G_i$ and prove that $P \cup M \cup \bigcup_i S_{G_i}$ is a resolving set of $G$ (Lemmas~\ref{toconclude},~\ref{structurecompM} and~\ref{iscode}).
    \item Bound the size of $M$ and $P$ as functions of $\tau$ and $c(G)$ (Lemmas ~\ref{boundN}, ~\ref{boundM},~\ref{boundMalt} and~\ref{boundP}).
    \item Prove the inequality $|\bigcup_i S_{G_i}| - \tau \leq Z(G)$  and conclude (Lemma~\ref{boundZ}).
\end{enumerate}


\subsection{Proof of Theorem~\ref{main}}

Let $J$ be the graph obtained from $G$ by an iterative deletion of vertices of degree $1$. Since $c \ge 2$, $J$ is not a cycle. 

Let $X \subseteq V$ be a feedback vertex set of $J$ such that each vertex of $X$ has at least degree three in $J$.

\begin{lemme}
Let $G$ be a connected graph with no vertex of degree $1$ that is not a cycle. There exists a feedback vertex set $X$ of size $\tau(G)$ with all vertices of $X$ of degree at least $3$.

\end{lemme}

\begin{proof}
Let $X$ be a minimum feedback vertex set with the minimum number of vertices of degree less than $3$. 
Assume by contradiction that $X$ contains a degree $2$ vertex $x$. Let $P$ be the maximal path of vertices of degree $2$ containing $x$. Since $G$ is not a cycle, $P$ does not contain the whole graph. Let $y$ be an endpoint of $P$. Let $X'=X \setminus \{x\} \cup \{y\}$. The set $X'$ is a feedback vertex set, a contradiction with the definition of $X$.  
%Assume there exists $Y \subseteq V$ such that $G \setminus Y$ is a forest and $|Y|<|X|$. Then, $H \setminus Y$ is also a forest. If $Y$ contains degree two vertices in $H$ then we move it to a path until reach a degree three vertex. This is possible as $H$ is not a cycle ($c \geq 2$). And this new set $Y'$ verify $|Y'|=|Y|$ and $H \setminus Y'$ is a forest as the moves on the vertices do not change the cycles they belong to. So $Y'$ satisfies the same condition than $X$ which is a contradiction as we assume $X$ has minimal size. 
\end{proof}

From now on we consider a minimum feedback vertex set $X$ of $G$ only containing vertices of degree at least $3$.
Let $G_1,G_2,...,G_k$ be the connected components of $G \setminus X$. Note that each $G_i$ induces a tree. For each $G_i$, let $X_i \subseteq X$ be the set of vertices of $X$ connected to at least one vertex of $G_i$. Let $N_i \subseteq V(G_i)$ be the set of vertices in $G_i$ adjacent to (at least) one vertex of $X_i$ and $E_i$ be the set of edges between $N_i$ and $X_i$. 

Let $T_i$ be the minimal subtree of $G_i$ containing the vertices of $N_i$. In other words, $T_i$ is the subtree of $G_i$ restricted to the union of the paths between $a$ and $b$ for any pair $a,b \in N_i$. Let $T'_i$ be the tree built from $T_i$ by adding to each vertex $u$ in $N_i$ as many leaves as $u$ have neighbors in $X$ in $G$. We define $M_i$ as the set of vertices in $T'_i$ of degree at least 3 in $T'_i$.
Let $M=X \cup (\bigcup_{i=1}^k M_i)$.

\begin{lemme}\label{structure}
For each connected component $H$ of $G \setminus M$ there are at most two edges in $G$ between $H$ and $G \setminus H$.
\end{lemme}
\begin{proof}
Let $U_H$ be the minimal subtree of $H$ containing all the vertices incident to an edge between $H$ and $G \setminus H$. Then, for each edge between a vertex $v \in H$ and a vertex in $G \setminus H$, add one new vertex in $U_H$ adjacent to $v$. Let us prove that if a vertex have degree at least 3 in $U_H$ then this vertex is in $M$. \\
Assume by contradiction $v \in U_H$ has degree 3 in $H$. Let $i$ be such that $H$ is a subgraph of $G_i$ and consider $T'_i$. The vertex $v$ is on a minimal path between two vertices of $M$ (otherwise $v \notin U_H$) so $v$ is also in $T'_i$ because the path in $G_i$ between these vertices is unique as $G_i$ is a tree. So the degree of $v$ is at least 3 in $T'_i$ and $v \in M$, a contradiction. 
\end{proof}

Lemma~\ref{structure} implies the following.

\begin{cor} 
Every connected component of $G \setminus M$ is connected to at most two vertices of $M$.
\end{cor}

A connected component of $G\setminus M$ can be attached to $M$ in three different ways, called {\em types}, that are illustrated in Figure~\ref{figexh}. A connected component has Type $A$ (respectively type $B$) if there are exactly two edges between $H$ and $M$ with distinct endpoints in $H$ and such that their endpoints in $M$ are distinct (resp. the same). A component $H$ has Type $C$ if all the edges of $G$ between $H$ and $M$ have the same endpoint in $H$ (but possibly distinct endpoints in $M$). 

Let $H$ be a connected component of $G \setminus M$ of type $A$ or $B$ and let $x$ and $y$ be the two endpoints in $M$ of the edges between $H$ and $M$. Let $\rho_H$ be one vertex on the path in $H$ between $x$ and $y$ such that $|d_H(x,\rho_H)-d_H(y,\rho_H)| \leq 1$. In other words, $\rho_H$ is one of the vertices in the middle of the path between $x$ and $y$ in $H$. Let $P$ be the union of the vertices $\rho_H$ for all the connected component $H$ of type $A$ and $B$.
 
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.6]{exh.pdf}
    \caption{The three types of components of $G\setminus M$.  }
    \label{figexh}
\end{figure}


\begin{lemme}\label{use_of_p}
Let $H$ be a connected component of $G \setminus M$ of type $A$ or $B$. Let $\rho$ be the vertex of $P \cap H$. Then, for any vertex $v \in H$, there is no shortest path between $z$ and $\rho$ using vertices in $G \setminus H$ and for $z \in \partial H$ there is a shortest path using only vertices in $H \cup \{z\}$.
\end{lemme}

\begin{proof}
Let $x$ and $y$ be the two vertices in $H$ adjacent to a vertex of $M$, $\alpha$ be the vertex of $M$ adjacent to $x$ and $\beta$ the vertex in $M$ adjacent to $y$. By definition of types $A$ or $B$, $x \neq y$ (but $\alpha$ and $\beta$ could be the same vertex if the type is $B$).

By definition of $\rho$, we have $|d_H(x,\rho)-d_H(y,\rho)| \leq 1$. Let $v \in V(H)$. Assume by contradiction that a shortest path between $v$ and $\rho$ in $G$ passes through vertices in $G \setminus H$. So this shortest path between $\rho$ and $v$ passes through $x$ and $y$. 
By symmetry we can assume $d_G(v,\rho)=d_H(v,x)+d(x,\alpha)+d(\alpha,\beta)+d(\beta,y)+d_H(y,\rho)$. In other words, the path from $v$ to $\rho$ passes through $x$ and then $y$.


Assume by contradiction that $d_H(z,x)+d(x,\alpha)+d(\alpha,\beta)+d(\beta,y)+d_H(y,\rho) \leq d_G(v,\rho)$. As $x\alpha$ and $y\beta$ are edges, we have $d_H(v,x)+d(\alpha,\beta)+d_H(y,\rho) +2 \leq d_G(v,\rho)$. By triangular inequality, $d_G(v,\rho) \leq d_H(v,\rho) \leq d_H(v,x)+d_H(x,\rho)$. So $d_H(x,\rho) \geq d_H(y,\rho)+d(\alpha,\beta)+2$ which contradicts $|d_H(x,\rho)-d_H(y,\rho)| \leq 1$. \\

If $z$ is in $\partial H$ and $\alpha=\beta$ then $z=\alpha=\beta$ and the result is immediate. Else assume $z=\alpha$ then we want to contradict $d(\alpha,\beta)+d(\beta,\rho) < d(\alpha,\rho)$. As $\alpha$ is adjacent to $x$ and $\beta$ adjacent to $y$ the inequality is equivalent to $d(\alpha,\beta) + d(y,\rho) < d(x,\rho)$. As $\alpha \neq \beta$, $d(\alpha,\beta) \geq 1$. So $d(y,\rho) +2 \leq d(x,\rho)$ which contradicts $|d_H(x,\rho)-d_H(y,\rho)| \leq 1$.
\end{proof}

We will now construct a resolving set of $G$. For every $i$, we define a metric basis $S_i$ of $G_i$ as follows. If $G_i$ is a path then $S_i$ is the extremity of the path the farthest to $X$. If $G_i$ is a branching tree then $S_i$ contains all but one terminal vertex for each major vertex on $G_i$. The set $S_i$ is a metric basis of $G[H_i]$ by Lemma~\ref{dimtree}. 
We will prove that $S_i$ resolves in $G$ the vertices inside the components of $G\setminus M$.
Let us first define the projection of a vertex.


\begin{defn}{}
Let $H$ be a connected component of $G \setminus M$ of type $A$ or $B$ and let $x$ and $y$ be the two vertices in $H$ adjacent to $M$. Let $u$ be any vertex of $H$. The \emph{projection $z_u$ of $u$ (on the path between $x$ and $y$)} is the unique vertex in the path between $x$ and $y$ in $H$ at minimum distance to $u$. %for $z \neq z_u$ and $z$ on the path between $x$ and $y$, $d(z,u)>d(z_u,u)$.
\end{defn}

\begin{lemme}\label{toconclude}

Let $H$ be a connected component of $G \setminus M$ of type $A$ or $B$. Let $u$ and $v$ be two vertices in $H$ and assume that a vertex $\gamma$ resolves the pair $(u,v)$ in $G_i$, the connected component of $G\setminus X$ that contains $H$. If $z_u=z_v$ then $\gamma$ resolves the pair $(u,v)$ in $G$.
\end{lemme}
\begin{proof}
We consider two cases $z_{\gamma}=z_u$ and $z_{\gamma} \neq z_u$.

If $z_{\gamma}=z_u=z_v$ then the distances to $\gamma$ are the same in $G_i$ and $G$: $d_{G_i}(\gamma,u)=d_G(\gamma,u)$ and $d_{G_i}(\gamma,v)=d_G(\gamma,v)$ so $d_G(\gamma,u) \neq d_G(\gamma,v)$ as $d_{G_i}(\gamma,u) \neq d_{G_i}(\gamma,v)$.

If $z_{\gamma} \neq z_u$ then $d_{G_i}(\gamma,u)=d_{G_i}(u,z_u)+d_{G_i}(z_u,\gamma)$ and $d_{G_i}(\gamma,v)=d_{G_i}(v,z_v)+d_{G_i}(z_v,\gamma)$. As $z_u=z_v$ and $d_{G_i}(\gamma,u) \neq d_{G_i}(\gamma,v)$, we have $d_{G_i}(u,z_u) \neq d_{G_i}(v,z_v)$. Since $d_{G_i}(u,z_u)=d_G(u,z_u)$ and $d_{G_i}(v,z_v)=d_G(v,z_v)$ we obtain $d_G(u,\gamma) \neq d_G(v,\gamma)$ since $d_G(u,\gamma)=d_G(u,z_u)+d_G(z_u,\gamma)$ and $d_G(v,\gamma)=d_G(v,z_v)+d_G(z_v,\gamma)$.
\end{proof}



\begin{lemme}\label{structurecompM}
Let $m$ be a vertex of $M$. Let $S= M \cup P \cup (\bigcup_i S_i)$. There is at most one connected component $H$ of $G \setminus M$ adjacent to $m$ and such that $H \cap S =\emptyset$. Moreover if such a component exists, it is a path with one extremity connected to $m$.
\end{lemme}
\begin{proof}
By definition of $P$, any connected component of type $A$ or $B$ contains an element of $P$. So the only connected components $H$ which can satisfy $H \cap S  =\emptyset$ are connected components $H$ of type $C$. 

Assume by contradiction that two connected components $H$ and $H'$ of $G \setminus M$ are connected to $m$  and that $H \cap S =\emptyset$ and $H' \cap S =\emptyset$.
If $m \in X$ then $H=G_i$ for some $i$. Since $S_i$ is a resolving set of $H$, $S_i$ is non empty and $H \cap S \neq \emptyset$. So we can assume that $m \in M \setminus X$. Thus $H$ and $H'$ are in the same connected component $G_i$ for some $i \in \{1,,\ldots,k\}$ since $m \notin X$ is connected to at least one vertex of $H$ and $H'$. If $S_i$ does not contain any vertex in $H \cup H'$ then the two vertices in $H \cup H'$ adjacent to $m$ are not resolving by $S_i$ in $G_i$ by Lemma~\ref{dimbranch}, a contradiction with the definition of $S_i$.

Let us now prove the second part of the statement. Let $H$ be a connected component of $G \setminus M$ connected to $w$ and such that  $H \cap S = \emptyset$. We have $H \subseteq G_i$ for some $i \in [1,k]$. Let $u$ be a terminal vertex in $H$ and consider the path between $u$ and $w$. Assume by contradiction this path contains vertex $v$ of degree $3$. Then, there exists a vertex $w$ adjacent to $v$ which is not on the path between $v$ and $m$ and a vertex $x$ adjacent to $u$ on the path between $u$ and $v$. The vertices $w$ and $x$ are not resolved by any vertex out of $H$ in $G_i$ so if $S_i \cap H= \emptyset$ there is a contradiction as $S_i$ is a resolving set of $G_i$. So the path between $v$ and $m$ contains only degree-2 vertices for any terminal vertex $v$ meaning $H$ is a path and $v$ the only terminal vertex of $H$.
\end{proof}

\begin{lemme} \label{iscode}
The set $S= M  \cup P \cup (\bigcup_i S_i) $ is a resolving set of $G$.
\end{lemme}

\begin{proof}
Assume by contradiction that $u$ and $v$ are different vertices at same distance to any vertex in $S$. Then, $u \notin M$ and $v \notin M$ as $M \subseteq S$. So there exist $H_u$ and $H_v$ connected components in $G \setminus M$ such that $u \in H_u$ and $v \in H_v$. \\
\begin{itemize}
\item Assume $H_u$ is of type $A$ and let $x\alpha$ and $y\beta$ be the two edges connecting $H_u$ to $M$ (with $x,y \in H_u$). Let $\rho$ be the vertex in $P \cap H_u$. Assume $v \notin H_u$. The shortest path between $v$ and $\rho$ passes through $\alpha$ or $\beta$. Assume by symmetry $\alpha$ is on the shortest path between $v$ and $\rho$ so $d(v,\rho)=d(v,\alpha)+d(\alpha,\rho)$. As $\alpha$ and $\rho$ are in $S$ we also have $d(u,\rho)=d(u,\alpha)+d(\alpha,\rho)$ which contradicts Lemma~\ref{use_of_p}. So $H_u=H_v$, denote it by $H$ from now and let $G_i$ be the component of $G\setminus X$ that contains $H$. \\
    
 The graph $H$ is a tree with a path between the two vertices $x$ and $y$.  We want to prove that $z_u=z_v$ by contradiction with $z_u$ and $z_v$ are defined in Lemma~\ref{use_of_p}. Assume it is not the case, without loss of generality we can assume $z_u \neq \rho$. 
 We have $d(u,\alpha)=d(u,z_u)+d(z_u,\alpha)$, $d(v,\alpha)=d(v,z_v)+d(z_v,\alpha)$, $d(u,\beta)=d(u,z_u)+d(z_u,\beta)$ and $d(v,\beta)=d(v,z_v)+d(z_v,\beta)$. As $d(u,\alpha)=d(v,\alpha)$ and $d(u,\beta)=d(v,\beta)$ we get \[d(z_u,\alpha)+d(z_v,\beta)=d(z_u,\beta)+d(z_v,\alpha)\]
    The vertices $z_u$ and $\rho$ are distinct and both between $\alpha$ and $\beta$ so $z_u$ is between $\alpha$ and $\rho$ or $\beta$ and $\rho$. Assume $z_u$ is between $\alpha$ and $\rho$ then $d(z_u,\alpha) \leq d(z_u,\beta)$ so $d(z_v,\alpha) \leq d(z_v,\beta)$ meaning $z_v$ is also between $\alpha$ and $\rho$.
    The shortest path between $\alpha$ and $\rho$ passes through $z_u$ and $z_v$ by Lemma~\ref{use_of_p}. 
    Assume $z_u$ is closer than $z_v$ to $\rho$ then $d(\alpha,\rho)=d(\alpha,z_v)+d(z_v,z_u)+d(z_u,\rho)$ gives 
    \[d(\alpha,z_u)+d(z_v,\rho)=d(\alpha,z_v)+d(z_u,\rho)+2d(z_u,z_v)\]
    Use now the paths to $\rho$: $d(u,\rho)=d(u,z_u)+d(z_u,\rho)$ as $z_u \neq \rho$ and $d(v,\rho) \leq d(v,z_v)+d(z_v,\rho)$ and reuse $d(u,\alpha)=d(u,z_u)+d(z_u,\alpha)$, $d(v,\alpha)=d(v,z_v)+d(z_v,\alpha)$ give 
    \[d(z_v,\alpha)+d(z_u,\rho) \leq d(z_u,\alpha)+d(z_v,\rho)\]
    Combine with the previous equality give $d(z_u,z_v) \leq 0$ so $z_u=z_v$. 
    
    The set $S$ contains $S_i$ which is a resolving set of $G_i$. So there exists $\gamma$ which resolves the pair $(u,v)$ in $G_i$ and thus resolves the pair $(u,v)$ in $G$ by Lemma~\ref{toconclude}.

  \item  Assume now that $H_u$ is of type $B$ and let $x\alpha$ and $y\beta$ be the two edges between $H_u$ and $M$.
    Let $\rho$ the vertex in $P \cap H_u$. If $v \notin H_u$ then $\alpha$ is on the path between $v$ and $\rho$ and $d(v,\rho)=d(v,\alpha)+d(\alpha,\rho)$ so $d(u,\rho)=d(u,\alpha)+d(\alpha,\rho)$ which contradicts Lemma~\ref{use_of_p}, so $H_u=H_v$. We denote $H_u=H_v$ as $H$ from now. \\
   We have $\alpha \in X$ as $H \cup \{\alpha\}$ contains a cycle. So $H=G_i$ for some $i \in [1,k]$.
    As $S$ contains $S_i$ which is a metric basis for $G_i$ if $u \neq v$ there exists $\gamma \in H$ such that $d_H(u,\gamma) \neq d_H(v,\gamma)$ and $d_G(u,\gamma) = d_G(v,\gamma)$. \\
    
    Assume first $z_{\gamma} = \rho$ and prove $\gamma$ resolves the pair $(u,v)$. Indeed if $z_{\gamma}=\rho$ we prove that $d_G(u,\gamma)=d_H(u,\gamma)$ and $d_G(v,\gamma)=d_H(v,\gamma)$. If $z_u=z_{\gamma}$ then $d_G(u,\gamma)=d_G(u,z_u)+d_G(z_u,\gamma)=d_H(u,z_u)+d_H(z_u,\gamma)=d_H(u,\gamma)$. If $z_u \neq z_{\gamma}$ then \[d_G(u,\gamma)=d_G(u,z_u)+d_G(z_u,\rho)+d_G(\rho,\gamma).\] By Lemma~\ref{use_of_p}, $d_G(z_u,\rho)=d_H(z_u,\rho)$. Thus $d_G(u,z_u)=d_H(u,z_u)$ because the path between these two vertices is unique. Similarly $d_G(\rho,\gamma)=d_H(\rho,\gamma)$. So $d_G(u,\gamma)=d_H(u,\gamma)$. In the same way, $d_G(v,\gamma)=d_H(v,\gamma)$ and $\gamma$ still resolves the pair $(u,v)$. \\
    
    Assume now $z_{\gamma} \neq \rho$. We have $d(u,\rho)=d(u,z_u)+d(z_u,\rho)$, $d(v,\rho)=d(v,z_v)+d(z_v,\rho)$, $d(u,\alpha)=d(u,z_u)+d(z_u,\alpha)$, $d(v,\alpha)=d(v,z_v)+d(z_v,\alpha)$, $d(u,\alpha)=d(v,\alpha)$ and $d(u,\rho)=d(v,\rho)$. Combine give \[d(z_u,\rho)+d(z_v,\alpha)=d(z_v,\rho)+d(z_u,\alpha)\] Moreover as $\rho$ and $\alpha$ are nearly opposed on the smallest cycle containing these two vertices we also have \[d(z_u,\rho)+d(z_u,\alpha)=d(z_v,\rho)+d(z_v,\alpha)+ \epsilon\] with $\epsilon \in \{-1,0,1\}$. Summing the two equalities give $2d(z_u,\rho)=2d(z_v,\rho)+ \epsilon$. So $\epsilon=0$, $d(z_u,\rho)=d(z_v,\rho)$ and $d(z_u,\alpha)=d(z_v,\alpha)$. Since  $d(u,\alpha)=d(v,\alpha)$, we obtain $d(u,z_u)=d(v,z_v)$.
    
    If $z_u \neq z_v$ then $z_u$ and $z_v$ are distinct and at the same distance to three points on a cycle ($\rho$, $\alpha$ and $z_\gamma$) which contradicts Lemma~\ref{cycle3}. If $z_u=z_v$ then Lemma~\ref{toconclude} allow use to conclude.
    
    \item Assume now that $H_u$ and $H_v$ are of type $C$. Let $\alpha$ and $\beta$ the vertices of $M$ connected to $H_u$ and $H_v$ respectively. If $\alpha \neq \beta$ then the shortest path between $u$ and $v$ contains two distinct vertices of $S$ so by Lemma~\ref{technical} $u$ and $v$ are resolved. Hence we assume that $\alpha=\beta$. \\
    We prove that $H_u=H_v$ by contradiction. If $H_u \neq H_v$,  by Lemma~\ref{structurecompM}, without loss of generality, there must exists $\gamma \in S \cap H_u$. If $u$ is on the path between $\gamma$ and $v$ then $d(\gamma,u) < d(\gamma,v)$.
    Otherwise let $m_u$ in $H_u$ be at the intersection of the path between $u$ and $\gamma$ and between $\alpha$ and $\gamma$. Then, vertices $m_u$ and $\alpha$ are on the shortest path between $u$ and $v$. By Lemma~\ref{technical}, one of them must resolve $u$ and $v$. By assumption, it is not $\alpha$. If it is $m_u$ then we would have $d_G(u,\gamma) \neq d_G(v,\gamma)$ since the shortest paths between $u$, $v$ and $\gamma$ go through $m_u$, a contradiction.
    \\
    Thus we can assume that $H_u=H_v$ and let $H=H_u$. Let $H\subseteq G_i$ for some $i$. The set $S_i$ resolves $u$ and $v$ in $G_i$. Let $\gamma\in S_i$ that resolves $u$ and $v$ in $G_i$. If $\gamma$ is in $H_u$, the  distances between $u$, $v$ and $\gamma$ in $G$ and $H$ are the same so $\gamma$ resolves $u$ and $v$. Otherwise, $d_H(u,\gamma)=d_H(u,x)+d_H(x,\gamma)$ where $x$ is the unique vertex of $H$ connected to the rest of the graph. Similarly, $d_H(v,\gamma)=d_H(v,x)+d(x,\gamma)$. Hence $d_H(u,x)\neq d_H(v,x)$ and thus since $d_G(u,\alpha)=d_H(u,x)+1$ and $d_G(v,\alpha)=d_H(u,x)+1$, $\alpha$ resolves $u$ and $v$.
    \end{itemize}
\end{proof}

 


 We now bound the size of the resolving set $S$. Recall that $E_i$ is the number of edges between $G_i$ and $X$. We use the following result on minors to get the bound.
 
 Let $G$ be a multigraph. The graph $H$ is a {\em minor} of $G$ if $H$ can be obtained from $G$ via a sequence of edge deletions, vertex deletions and edge contractions (the edge contraction operation can create parallel edges between two vertices or loops). One can easily check that the minor operation can only decrease the cycle rank.\\
\begin{lemme} \label{boundN}
$\sum_{i=1}^k (|E_i|-1) \leq c+\tau-1 $.
\end{lemme}
\begin{proof}
Let $G'$ be a multigraph obtained from $G$ by contracting all the connected components $G_i$ into one vertex $v_i$. Since $G'$ is a minor of $G$, $c(G') \leq c(G)$ and $G'$ is still connected since we have not deleted edges. The graph $G'$ contains $\tau+k$ vertices so $G'$ contains at most $c(G)+\tau+k-1$ edges.
So $\sum_{i=1}^k |E_i| \leq c+\tau+k-1 $ and $\sum_{i=1}^k (|E_i|-1) \leq c+\tau-1 $.
\end{proof}

In the next two lemmas, we give two bounds on the size of $M$ (one depending only of $c$ and the other of $\tau$ and $c$). . Recall that $T_i$ is the minimal subtree of $G_i$ containing the vertices of $N_i$ and $T'_i$ is the tree built from $T_i$ by adding to each vertex $u$ in $N_i$ as many leaves as $u$ have neighbors in $X$ in $G$. 


\begin{lemme}\label{boundM}
$|M| \leq c+2\tau-2$.
\end{lemme}
\begin{proof}
Consider a subgraph $G_i$ of $G$ such that $|M \cap G_i| \neq \emptyset$ , we want to prove that $|M \cap G_i| \leq |E_i|-2$ and use Lemma~\ref{boundN}.

If $|E_i| \leq 2$ then  $M \cap G_i = \emptyset$ since $T_i'$ is reduced to a path and then has no degree-$3$ vertex.
So we can assume that $|E_i| \geq 3$. By construction, $T_i'$ contains $|E_i|$ leaves and then at most $|E_i|-2 $ vertices of degree at least 3. 
Indeed let $T$ be any tree on $n$ vertices with $k_1$ leaves, $k_2$ degree-$2$ vertices, and $k_3$ vertices with degree at least $3$. The sum of the degree of all the vertices is $2n - 2$ ($T$ being connected). Thus $k_1 + 2k_2 + 3k_3 \leq 2n - 2$ and then, $k_1 + 3k_3 \leq 2n - 2 - 2k_2 = 2(k_1+k_2+k_3) -2 -2k_2 $. So $k_1 + 3k_3 \leq  2(k_1 + k_3) - 2$. That gives $k_3 \leq k_1 - 2$ which is the target.

Since the vertices in $M \cap G_i$ are the vertices of degree at least $3$ in $T_i'$, we have $|M \cap G_i| \leq |E_i|-2$. Since $M=X \cup (\bigcup_{i=1}^k M_i)$, summing on all the $G_i$ with $M \cap G_i \neq \emptyset$ gives $|M| \leq \tau + \sum_{G_i, M \cap G_i \neq \emptyset} (|E_i|-2) $.
So we have:
\[|M| \leq \tau+ \sum_{G_i, M \cap G_i \neq \emptyset} (|E_i|-2) \leq \tau +\sum_{G_i, M \cap G_i \neq \emptyset} (|E_i|-1) - |\{i,  M \cap G_i \neq \emptyset\}|\]
By Lemma~\ref{boundN}, $\sum_{G_i, M \cap G_i \neq \emptyset} (|E_i|-1) \leq \sum_{G_i} (|E_i|-1) \leq c + \tau -1$. Since $|\{i,  M \cap G_i \neq \emptyset\}| \ge 1$ (otherwise $|M|=0$ and the conclusion holds) gives $|M| \leq c+2\tau-2$.
\end{proof}

\begin{lemme}\label{boundMalt}
$|M| \leq 2c-2$. 
\end{lemme}
\begin{proof}

If $|M|\leq 2$ then the inequality holds since $c \geq 2$. So we can assume that $|M| \ge 3$. Let $K$ be the multigraph (with possible loops) with vertex set $M$ where, for each connected component $H$ of $G \setminus M$ of type $A$ or $B$ with endpoints $x$ and $y$ in $M$ (that might be identical), we create an edge between $x$ and $y$ in $K$. Note that $K$ is a minor of $G$ as it can be obtained from $G$ by contracting edges in components $H$ of $G \setminus M$ into a single edge.

Every vertex in $K$ has degree at least $3$. The vertices of $M\setminus X$ has degree at least $3$ by definition of $M_i$ for every $i$. 
By construction of $X$, $x \in X$ has degree at least three in the graph starting from $G$ and removing the degree one vertices. The three adjacent edges all contribute to the degree of $x$ in $K$ so $\deg_{K}(x) \geq 3$.

We have $3 |V(K)| \le \sum_{v \in V(K)} \deg(v) = 2 |E(K)|$. So $3|M| \leq 2 |E|$. And the cycle rank of $K$ is at most $c$, so $|E| \leq c + |M| - 1 $. A combination of these inequalities gives $|M| \leq 2c-2$.
\end{proof}


\begin{lemme}\label{boundP}
$|P| \leq c + |M|-1$.
\end{lemme}
\begin{proof}
Let $K'$ be the multigraph (with loops) with vertex set $M$ and an edge between two vertices $x$ and $y$ if and only if there exists in $G \setminus M$ a connected component $H$ adjacent to $x$ and $y$. The graph $K'$ is a minor of $G$ since $K'$ can be obtained from $G$ by contracting edges with exactly one endpoint in $M$ until no such edge exists. One can easily notice that $K'$ there is an edge $xy$ with multiplicity $k$ if and only if in $G \setminus M$ there are $k$ connected components attached to $x$ and $y$. 
Since $K'$ is a minor of $G$, $c(K') \leq c(G)$. As $K'$ contains $|M|$ vertices it contains at most $c+|M|-1$ edges. Since $P$ contains one vertex in each component of type A or B, we have $|P| \leq c+|M|-1$.
\end{proof}


\begin{lemme} \label{boundZ}
$|\bigcup_i S_i| - \tau \leq Z(G)$.
\end{lemme}
\begin{proof}
Let $Z$ be a minimal zero forcing set for $G$. Let $\mathcal{S}$ be a sequence of forcings that turns $G$ into black starting from $Z$. Let $Z'$ be the set of vertices turned black in $\mathcal{S}$ because of a vertex of $X$. Note that $|Z'| \le \tau$.
Let $G_i$ be a connected component of $G[V \setminus X]$. We claim that $(Z \cup Z') \cap V(G_i)$ is a zero-forcing set of $G_i$. If we restrict the sequence of colorings that turn $G$ to black from $Z$, then this sequence also works in $G_i'$. A vertex always has at most as many white neighbors as in $G$. So the only problem that can appear is that a vertex $v$ would have to be turned black because of $u$ in $G$ and $u \notin V(G_i)$. But the only vertices not in $V(G_i)$ that can turn black vertices of $G_i$ are the vertices of $X$. Therefore vertices turned black because of $X$ are in $Z' \cap V(G_i)$ and then are already black.

So, by Lemma~\ref{treecomp}, we have $|S_{G_i}| \leq |Z' \cap G_i|$. When we consider the union over all the components, it gives $ |Z \cup Z'| \ge \cup_i |S_{G_i}|$. Since $Z'$ has size at most $\tau$, we have  $ Z(G) \geq |\bigcup_i S_{G_i}| - \tau $.
%Let $Z$ be a minimal zero forcing set for $G$, we add (at most) $|X|$ vertices to $Z$ to get a set $Z'$ such that for all components $G_i$ of $G \setminus X$, $Z'\cap G_i$ is a forcing set of $G_i$.
%To define the vertices consider a sequence for coloring in $G$ starting from $Z$. Let $Z'$ be equal to $Z$ union the vertices turned black by one vertex of $X$. As a vertex can colored at most one other vertex we have $|Z'| \leq |Z|+|X|$. The property announced for $Z'$ hold because for $G_i$ a connected component, $Z' \cap G_i$ is a forcing set because all the same sequences than in $G$ are still valid in $Z \cap G_i$. 
%For $G_i$ a connected component $S_i$ is a basis for $G_i$ so $|S_{G_i}| \leq |Z' \cap G_i|$. Take the union give
%$ |Z'| \geq \sum_{i} |Z' \cap G_i| \geq |\bigcup_i S_{G_i}|  $. So $ Z(G) \geq |\bigcup_i S_{G_i}| - |X| $.
\end{proof}

We can now conclude.
\begin{proof}[Proof of Theorem~\ref{main}]
We know that $S= M \cup P \cup (\bigcup_i S_{G_i}) $ is a resolving set of $G$ so $\dim(G) \leq |S|$. Moreover $ Z(G) \geq |\bigcup_i S_{G_i}| - \tau $. That give $\dim(G) \leq |M|+|P|+\tau+Z(G) $. So we get $\dim(G) \leq 2|M|+c+\tau-1+ Z(G)$. We bound $|M|$ by $c+2\tau-2$ and by $2c-2$ so $\dim(G) \leq  Z(G) + \min(5c+\tau-5,3c+5\tau-5)$.
\end{proof}


